A Benchmarking of QCD Evolution at Approximate $N^3LO$

We present a detailed benchmarking of different treatments of the QCD evolution of unpolarized PDFs at approximate $N^3LO$ ($aN^3LO$) order in the QCD coupling. Namely, the implementations in the public $aN^3LO$ releases of the MSHT and NNPDF global PDF fitters, as well as that of the theoretical FHMRUVV collaboration are compared. This follows the same procedure as in previous benchmarking exercises at lower order, that is by considering the impact of this evolution on a set of simple toy PDFs.

==> tables/lo_bench.tex <==
\begin{table}[htp]
\caption{Reference results for the $n_f=4$ (FFN) and the 
  variable-$n_f$ (VFN) leading-order evolution for the initial conditions
  and the input parton distributions 
  in Eqs.~(\ref{eq:muf-start})), (\ref{eq:input}) and (\ref{eq:alphas-start}).
 The respective values for $\alpha_{\rm s}(\mu_{\rm r}^2\! =\! \mu_{\rm f}^2\! =\! 10^4 \mbox{ GeV}^2)$ read $0.117374$ 
 (FFN) and $0.122306$ (VFN).} 
\label{tab:lo_benc}
%
\begin{center}
\vspace{5mm}
\begin{tabular}{||c||r|r|r|r|r|r|r|r||}
\hline \hline
\multicolumn{9}{||c||}{} \\[-3mm]
\multicolumn{1}{||c||}{$x$} &
\multicolumn{1}{c|} {$xu_v$} &
\multicolumn{1}{c|} {$xd_v$} &
\multicolumn{1}{c|} {$xL_-$} &
\multicolumn{1}{c|} {$xL_+$} &
\multicolumn{1}{c|} {$xs_+$} &
\multicolumn{1}{c|} {$xc_+$} &
\multicolumn{1}{c|} {$xb_+$} &
\multicolumn{1}{c||}{$xg$} \\[0.5mm] \hline \hline
\multicolumn{9}{||c||}{} \\[-3mm]
\multicolumn{9}{||c||}{Input, $\,\mu_{\rm f}^2 = 2 \mbox{ GeV}^2$} \\
\multicolumn{9}{||c||}{} \\[-0.3cm] \hline \hline
 & & & & & & & \\[-0.3cm]
$\! 10^{-7}\!$ &
$\! 1.2829^{-5}\!$ &$\! 7.6972^{-6}\!$ &$\! 9.7224^{-8}\!$ &$\! 3.8890^{+0}\!$ &
$\! 7.7779^{-1}\!$ &$\! 0.0   ^{+0}\!$ &$\! 0.0   ^{+0}\!$ &$\! 8.5202^{+0}\!$\\
$\! 10^{-6}\!$ &
$\! 8.0943^{-5}\!$ &$\! 4.8566^{-5}\!$ &$\! 7.7227^{-7}\!$ &$\! 3.0891^{+0}\!$ &
$\! 6.1782^{-1}\!$ &$\! 0.0   ^{+0}\!$ &$\! 0.0   ^{+0}\!$ &$\! 6.7678^{+0}\!$\\
$\! 10^{-5}\!$ &
$\! 5.1070^{-4}\!$ &$\! 3.0642^{-4}\!$ &$\! 6.1341^{-6}\!$ &$\! 2.4536^{+0}\!$ &
$\! 4.9072^{-1}\!$ &$\! 0.0   ^{+0}\!$ &$\! 0.0   ^{+0}\!$ &$\! 5.3756^{+0}\!$\\
$\! 10^{-4}\!$ &
$\! 3.2215^{-3}\!$ &$\! 1.9327^{-3}\!$ &$\! 4.8698^{-5}\!$ &$\! 1.9478^{+0}\!$ &
$\! 3.8957^{-1}\!$ &$\! 0.0   ^{+0}\!$ &$\! 0.0   ^{+0}\!$ &$\! 4.2681^{+0}\!$\\
$\! 10^{-3}\!$ &
$\! 2.0271^{-2}\!$ &$\! 1.2151^{-2}\!$ &$\! 3.8474^{-4}\!$ &$\! 1.5382^{+0}\!$ &
$\! 3.0764^{-1}\!$ &$\! 0.0   ^{+0}\!$ &$\! 0.0   ^{+0}\!$ &$\! 3.3750^{+0}\!$\\
$\! 10^{-2}\!$ &
$\! 1.2448^{-1}\!$ &$\! 7.3939^{-2}\!$ &$\! 2.8946^{-3}\!$ &$\! 1.1520^{+0}\!$ &
$\! 2.3041^{-1}\!$ &$\! 0.0   ^{+0}\!$ &$\! 0.0   ^{+0}\!$ &$\! 2.5623^{+0}\!$\\
$\! 0.1    \!$ &
$\! 5.9008^{-1}\!$ &$\! 3.1864^{-1}\!$ &$\! 1.2979^{-2}\!$ &$\! 4.9319^{-1}\!$ &
$\! 9.8638^{-2}\!$ &$\! 0.0   ^{+0}\!$ &$\! 0.0   ^{+0}\!$ &$\! 1.2638^{+0}\!$\\
$\! 0.3    \!$ &
$\! 6.6861^{-1}\!$ &$\! 2.8082^{-1}\!$ &$\! 7.7227^{-3}\!$ &$\! 8.7524^{-2}\!$ &
$\! 1.7505^{-2}\!$ &$\! 0.0   ^{+0}\!$ &$\! 0.0   ^{+0}\!$ &$\! 3.2228^{-1}\!$\\
$\! 0.5    \!$ &
$\! 3.6666^{-1}\!$ &$\! 1.1000^{-1}\!$ &$\! 1.6243^{-3}\!$ &$\! 9.7458^{-3}\!$ &
$\! 1.9492^{-3}\!$ &$\! 0.0   ^{+0}\!$ &$\! 0.0   ^{+0}\!$ &$\! 5.6938^{-2}\!$\\
$\! 0.7    \!$ &
$\! 1.0366^{-1}\!$ &$\! 1.8659^{-2}\!$ &$\! 1.0259^{-4}\!$ &$\! 3.8103^{-4}\!$ &
$\! 7.6207^{-5}\!$ &$\! 0.0   ^{+0}\!$ &$\! 0.0   ^{+0}\!$ &$\! 4.2810^{-3}\!$\\
$\! 0.9    \!$ &
$\! 4.6944^{-3}\!$ &$\! 2.8166^{-4}\!$ &$\! 1.7644^{-7}\!$ &$\! 4.3129^{-7}\!$ &
$\! 8.6259^{-8}\!$ &$\! 0.0   ^{+0}\!$ &$\! 0.0   ^{+0}\!$ &$\! 1.7180^{-5}\!$\\
%
\hline \hline
%
\multicolumn{9}{||c||}{} \\[-3mm]
\multicolumn{9}{||c||}{LO, $\, n_f = 4\,$, 
                       $\,\mu_{\rm f}^2 = 10^4 \mbox{ GeV}^2$} \\
\multicolumn{9}{||c||}{} \\[-0.3cm] \hline \hline
 & & & & & & & \\[-0.3cm]
$\! 10^{-7}\!$ &
$\! 5.7722^{-5}\!$ &$\! 3.4343^{-5}\!$ &$\! 7.6527^{-7}\!$ &$\! 9.9465^{+1}\!$ &
$\! 4.8642^{+1}\!$ &$\! 4.7914^{+1}\!$ &$\! 0.0   ^{+0}\!$ &$\! 1.3162^{+3}\!$\\
$\! 10^{-6}\!$ &
$\! 3.3373^{-4}\!$ &$\! 1.9800^{-4}\!$ &$\! 5.0137^{-6}\!$ &$\! 5.0259^{+1}\!$ &
$\! 2.4263^{+1}\!$ &$\! 2.3685^{+1}\!$ &$\! 0.0   ^{+0}\!$ &$\! 6.0008^{+2}\!$\\
$\! 10^{-5}\!$ &
$\! 1.8724^{-3}\!$ &$\! 1.1065^{-3}\!$ &$\! 3.1696^{-5}\!$ &$\! 2.4378^{+1}\!$ &
$\! 1.1501^{+1}\!$ &$\! 1.1042^{+1}\!$ &$\! 0.0   ^{+0}\!$ &$\! 2.5419^{+2}\!$\\
$\! 10^{-4}\!$ &
$\! 1.0057^{-2}\!$ &$\! 5.9076^{-3}\!$ &$\! 1.9071^{-4}\!$ &$\! 1.1323^{+1}\!$ &
$\! 5.1164^{+0}\!$ &$\! 4.7530^{+0}\!$ &$\! 0.0   ^{+0}\!$ &$\! 9.7371^{+1}\!$\\
$\! 10^{-3}\!$ &
$\! 5.0392^{-2}\!$ &$\! 2.9296^{-2}\!$ &$\! 1.0618^{-3}\!$ &$\! 5.0324^{+0}\!$ &
$\! 2.0918^{+0}\!$ &$\! 1.8089^{+0}\!$ &$\! 0.0   ^{+0}\!$ &$\! 3.2078^{+1}\!$\\
$\! 10^{-2}\!$ &
$\! 2.1955^{-1}\!$ &$\! 1.2433^{-1}\!$ &$\! 4.9731^{-3}\!$ &$\! 2.0433^{+0}\!$ &
$\! 7.2814^{-1}\!$ &$\! 5.3247^{-1}\!$ &$\! 0.0   ^{+0}\!$ &$\! 8.0546^{+0}\!$\\
$\! 0.1    \!$ &
$\! 5.7267^{-1}\!$ &$\! 2.8413^{-1}\!$ &$\! 1.0470^{-2}\!$ &$\! 4.0832^{-1}\!$ &
$\! 1.1698^{-1}\!$ &$\! 5.8864^{-2}\!$ &$\! 0.0   ^{+0}\!$ &$\! 8.8766^{-1}\!$\\
$\! 0.3    \!$ &
$\! 3.7925^{-1}\!$ &$\! 1.4186^{-1}\!$ &$\! 3.3029^{-3}\!$ &$\! 4.0165^{-2}\!$ &
$\! 1.0516^{-2}\!$ &$\! 4.1379_*^{-3}\!$&$\!0.0   ^{+0}\!$ &$\! 8.2676^{-2}\!$\\
$\! 0.5    \!$ &
$\! 1.3476^{-1}\!$ &$\! 3.5364^{-2}\!$ &$\! 4.2815^{-4}\!$ &$\! 2.8624^{-3}\!$ &
$\! 7.3137^{-4}\!$ &$\! 2.6481^{-4}\!$ &$\! 0.0   ^{+0}\!$ &$\! 7.9240^{-3}\!$\\
$\! 0.7    \!$ &
$\! 2.3123^{-2}\!$ &$\! 3.5943^{-3}\!$ &$\! 1.5868^{-5}\!$ &$\! 6.8961^{-5}\!$ &
$\! 1.7725^{-5}\!$ &$\! 6.5549^{-6}\!$ &$\! 0.0   ^{+0}\!$ &$\! 3.7311^{-4}\!$\\
$\! 0.9    \!$ &
$\! 4.3443^{-4}\!$ &$\! 2.2287^{-5}\!$ &$\! 1.1042^{-8}\!$ &$\! 3.6293^{-8}\!$ &
$\! 1.0192^{-8}\!$ &$\! 4.8893_*^{-9}\!$&$\!0.0   ^{+0}\!$ &$\! 1.0918^{-6}\!$\\
%
\hline \hline
%
\multicolumn{9}{||c||}{} \\[-3mm]
\multicolumn{9}{||c||}{LO, $\, n_f = 3\ldots 5\,$, 
                        $\,\mu_{\rm f}^2 = 10^4 \mbox{ GeV}^2$} \\
\multicolumn{9}{||c||}{} \\[-0.3cm] \hline \hline
 & & & & & & & \\[-0.3cm]
$\! 10^{-7}\!$ &
$\! 5.8771^{-5}\!$ &$\! 3.4963^{-5}\!$ &$\! 7.8233^{-7}\!$ &$\! 1.0181^{+2}\!$ &
$\! 4.9815^{+1}\!$ &$\! 4.9088^{+1}\!$ &$\! 4.6071^{+1}\!$ &$\! 1.3272^{+3}\!$\\
$\! 10^{-6}\!$ &
$\! 3.3933^{-4}\!$ &$\! 2.0129^{-4}\!$ &$\! 5.1142^{-6}\!$ &$\! 5.1182^{+1}\!$ &
$\! 2.4725^{+1}\!$ &$\! 2.4148^{+1}\!$ &$\! 2.2239^{+1}\!$ &$\! 6.0117^{+2}\!$\\
$\! 10^{-5}\!$ &
$\! 1.9006^{-3}\!$ &$\! 1.1229^{-3}\!$ &$\! 3.2249^{-5}\!$ &$\! 2.4693^{+1}\!$ &
$\! 1.1659^{+1}\!$ &$\! 1.1201^{+1}\!$ &$\! 1.0037^{+1}\!$ &$\! 2.5282^{+2}\!$\\
$\! 10^{-4}\!$ &
$\! 1.0186^{-2}\!$ &$\! 5.9819^{-3}\!$ &$\! 1.9345^{-4}\!$ &$\! 1.1406^{+1}\!$ &
$\! 5.1583^{+0}\!$ &$\! 4.7953^{+0}\!$ &$\! 4.1222^{+0}\!$ &$\! 9.6048^{+1}\!$\\
$\! 10^{-3}\!$ &
$\! 5.0893^{-2}\!$ &$\! 2.9576^{-2}\!$ &$\! 1.0730^{-3}\!$ &$\! 5.0424^{+0}\!$ &
$\! 2.0973^{+0}\!$ &$\! 1.8147^{+0}\!$ &$\! 1.4582^{+0}\!$ &$\! 3.1333^{+1}\!$\\
$\! 10^{-2}\!$ &
$\! 2.2080^{-1}\!$ &$\! 1.2497^{-1}\!$ &$\! 4.9985^{-3}\!$ &$\! 2.0381^{+0}\!$ &
$\! 7.2625^{-1}\!$ &$\! 5.3107^{-1}\!$ &$\! 3.8106^{-1}\!$ &$\! 7.7728^{+0}\!$\\
$\! 0.1    \!$ &
$\! 5.7166^{-1}\!$ &$\! 2.8334^{-1}\!$ &$\! 1.0428^{-2}\!$ &$\! 4.0496^{-1}\!$ &
$\! 1.1596^{-1}\!$ &$\! 5.8288^{-2}\!$ &$\! 3.5056^{-2}\!$ &$\! 8.4358^{-1}\!$\\
$\! 0.3    \!$ &
$\! 3.7597^{-1}\!$ &$\! 1.4044^{-1}\!$ &$\! 3.2629^{-3}\!$ &$\! 3.9592^{-2}\!$ &
$\! 1.0363^{-2}\!$ &$\! 4.0740^{-3}\!$ &$\! 2.2039^{-3}\!$ &$\! 7.8026^{-2}\!$\\
$\! 0.5    \!$ &
$\! 1.3284^{-1}\!$ &$\! 3.4802^{-2}\!$ &$\! 4.2031^{-4}\!$ &$\! 2.8066^{-3}\!$ &
$\! 7.1707^{-4}\!$ &$\! 2.5958^{-4}\!$ &$\! 1.3522^{-4}\!$ &$\! 7.4719^{-3}\!$\\
$\! 0.7    \!$ &
$\! 2.2643^{-2}\!$ &$\! 3.5134^{-3}\!$ &$\! 1.5468^{-5}\!$ &$\! 6.7201^{-5}\!$ &
$\! 1.7278^{-5}\!$ &$\! 6.3958^{-6}\!$ &$\! 3.3996^{-6}\!$ &$\! 3.5241^{-4}\!$\\
$\! 0.9    \!$ &
$\! 4.2047^{-4}\!$ &$\! 2.1529^{-5}\!$ &$\! 1.0635^{-8}\!$ &$\! 3.4998^{-8}\!$ &
$\! 9.8394^{-9}\!$ &$\! 4.7330^{-9}\!$ &$\! 2.8903^{-9}\!$ &$\! 1.0307^{-6}\!$\\
%
\hline \hline
%
\end{tabular}
\end{center}
\end{table}
